A Computational Note on the Application of the Supplemented EM Algorithm to Item Response Models

The EM algorithm is a method for finding the maximum likelihood estimate of a model in the presence of missing data. Unfortunately, EM does not produce a parameter covariance matrix for standard errors. Supplemented EM (SEM; Meng & Rubin, 1991) is one method for obtaining the parameter covariance matrix. SEM is implemented in both open-source (e.g., Chalmers, 2012; Pritikin, Hunter, & Boker, 2015) and commercial (e.g., Cai, Thissen, & du Toit, 2011) item response model estimation software. However, the original formulation of SEM did not adequately account for the limitations of IEEE 754 floating-point. Agile-SEM, a novel refinement of SEM, is proposed and compared against the original algorithm and a recent refinement (Tian, Cai, Thissen, & Xin, 2013) in a variety of item response model simulation studies. By controlling for the numerical noise intensity on a per-parameter basis, Agile-SEM demonstrated the best convergence properties, accuracy, and efficiency while, at the same time, requiring fewer tuning parameters. Complete source code is made freely available. The potential generalization of Agile-SEM to other EM application besides item response models is left as future work.

==> hylatex.ltx <==
%
% hylatex.ltx
% Tanmoy Bhattacharya and Sebastian Rahtz, June 1995
%
% Use this file to make a format which includes the
% hyperref package in every LaTeX job.
%
% In web2c 7-based TeX world, we create the format file with
%   tex  -ini \&latex hylatex.ltx
% and then use with
%   tex \&hylatex
%
% In teTeX (TeX version 3.14159 (C version 6.1), LaTeX2e <1996/12/01>
% patch level 1), I create the format file with
%   initex \&latex hylatex.ltx
% and then use with
%   virtex \&hylatex
%
% This method is not supported by the LaTeX2e team, so
% I will try to find a better way. \AtBeginDocument does not
% work for reasons which I do not understand.
%
\makeatletter
\expandafter\everyjob\expandafter{\the\everyjob
 \typeout{ ********* Hyperref Macros loaded ******* }}
%
\expandafter\let\csname REAL document\endcsname\document
%
\def\document{%
 \endgroup
%
% NOTE:
% This setup sets up no options by default;
% change to suit your needs, by writing a hyperref.cfg control
% file.
%
 \RequirePackage{hyperref}
 \begingroup
 \@endpefalse\csname REAL document\endcsname
}
\makeatother
\dump


